Flower: A Friendly Federated Learning Research Framework

Federated Learning (FL) has emerged as a promising technique for edge devices to collaboratively learn a shared prediction model, while keeping their training data on the device, thereby decoupling the ability to do machine learning from the need to store the data in the cloud. However, FL is difficult to implement realistically, both in terms of scale and systems heterogeneity. Although there are a number of research frameworks available to simulate FL algorithms, they do not support the study of scalable FL workloads on heterogeneous edge devices. In this paper, we present Flower -- a comprehensive FL framework that distinguishes itself from existing platforms by offering new facilities to execute large-scale FL experiments and consider richly heterogeneous FL device scenarios. Our experiments show Flower can perform FL experiments up to 15M in client size using only a pair of high-end GPUs. Researchers can then seamlessly migrate experiments to real devices to examine other parts of the design space. We believe Flower provides the community with a critical new tool for FL study and development.

==> diagrams/figure1.tex <==
% TIKZ PICTURE ----------------------------

\begin{figure}[!t]
\centering
\hspace{-1cm}
\scalebox{0.7}{
\begin{tikzpicture}
\begin{axis}[
    ybar,
    ylabel near ticks,
    enlargelimits=0.15,
    legend style={at={(0.5,-0.15)},
      anchor=north,legend columns=-1},
    ylabel={\# papers},
    xlabel={Total \# clients},
    symbolic x coords={$<$10,100,1k,10k,100k,1M,$>$1M},
    xtick=data,
    nodes near coords,
    nodes near coords align={vertical},
    ]
\addplot coordinates {($<$10,35)(100,87)(1k,15)(10k,9)(100k,1)(1M,3)($>$1M,0)};

%\legend{used,understood,not understood}
\end{axis}
\end{tikzpicture}
}
\caption{Survey of the number of FL clients used in FL research papers in the last two years. A vast majority of papers only use up to 100 clients. Appendix~\ref{appendix:paper-scale} gives details of the papers considered.}
\label{fig:maxclients}
\vspace{-0.5cm}
\end{figure}


==> sections/amazon_books.tex <==
\subsection{Amazon Review Dataset - Books}
The Amazon Review Dataset contains over 51M book reviews.
In our experiments partitions were

==> sections/communication.tex <==

\begin{tikzpicture}[scale=0.60]
\begin{axis}[align =center,
    title={},
    xlabel={Model vector size},
    ylabel={Data transferred (100 MB)},
    xlabel near ticks,
    ylabel near ticks,
    xmin=0, xmax=600000,
    ymin=0, ymax=20,
    xtick={0,100000,200000,300000,400000,500000},
    ytick={0,5,10, 15,20},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=blue,
    mark=*
    ]
    coordinates {
    (100000,10.03374636)(200000,10.83374636)(300000, 11.63375036)(400000,12.43375036)(500000,13.23375036)
    };
    
    
\addplot[
    color=red,
    mark=*
    ]
    coordinates {
    (100000,10.03492441)(200000,10.83492441)(300000,11.63492841)(400000, 12.43492841)(500000, 13.23492841)
    };
    \legend{0\% dropout,5\% dropout}
    
\end{axis}
\end{tikzpicture}


==> sections/femnist.tex <==
\subsection{FEMNIST Dataset}
Federated Extended MNIST (FEMNIST) \cite{caldas2018leaf} is built by partitioning the data in Extended MNIST \cite{cohen2017emnist} based on the writer of the digit/character. To replicate the experiments in \cite{caldas2018leaf}, we used the exactly same parameters to generate the experimental subset (0.05 fraction) of FEMNIST with fixed seeds for data sampling and splitting. Concretely, the data was sampled in a non-IID manner with minimum $100$ samples per user.

